AI on AI: Exploring the Utility of GPT as an Expert Annotator of AI Publications

Identifying scientific publications that are within a dynamic field of research often requires costly annotation by subject-matter experts. Resources like widely-accepted classification criteria or field taxonomies are unavailable for a domain like artificial intelligence (AI), which spans emerging topics and technologies. We address these challenges by inferring a functional definition of AI research from existing expert labels, and then evaluating state-of-the-art chatbot models on the task of expert data annotation. Using the arXiv publication database as ground-truth, we experiment with prompt engineering for GPT chatbot models to identify an alternative, automated expert annotation pipeline that assigns AI labels with 94% accuracy. For comparison, we fine-tune SPECTER, a transformer language model pre-trained on scientific publications, that achieves 96% accuracy (only 2% higher than GPT) on classifying AI publications. Our results indicate that with effective prompt engineering, chatbots can be used as reliable data annotators even where subject-area expertise is required. To evaluate the utility of chatbot-annotated datasets on downstream classification tasks, we train a new classifier on GPT-labeled data and compare its performance to the arXiv-trained model. The classifier trained on GPT-labeled data outperforms the arXiv-trained model by nine percentage points, achieving 82% accuracy.

==> 0_abstract/0_abstract.tex <==
\begin{abstract}
    Identifying scientific publications that are within a dynamic field of research often requires costly annotation by subject-matter experts.
    % is there better single word than dynamic?
    %
    % is most tractable given widely-accepted criteria for relevance, or a comprehensive taxonomy of the field. 
    %
    Resources like widely-accepted classification criteria or field taxonomies are unavailable for a domain like artificial intelligence (AI), which spans emerging topics and technologies.
    %
    % The best available source of ground truth 
    % This is one example of a 
    %
    We address these challenges by inferring a functional definition of AI research from existing expert labels, and then evaluating state-of-the-art chatbot models on the task of expert data annotation. Using the arXiv publication database as ground-truth, we experiment with prompt engineering for GPT chatbot models to identify an alternative, automated expert annotation pipeline that assigns AI labels with 94\% accuracy. For comparison, we fine-tune SPECTER, a transformer language model pre-trained on scientific publications, that achieves 96\% accuracy (only 2\% higher than GPT) on classifying AI publications. Our results indicate that with effective prompt engineering, chatbots can be used as reliable data annotators even where subject-area expertise is required. To evaluate the utility of chatbot-annotated datasets on downstream classification tasks, we train a new classifier on GPT-labeled data and compare its performance to the arXiv-trained model. The classifier trained on GPT-labeled data outperforms the arXiv-trained model by nine percentage points, achieving 82\% accuracy. 
    
    %Generating a dataset of GPT-labeled AI publications, we compare both classifiers on a set of publications from the top 13 AI conference venues to evaluate the utility of chatbots as data annotators for downstream tasks. 
    
   % train a baseline AI publication classifier with the SPECTER transformer language model that achieves 96\% accuracy.
    %
    %Leveraging expert-labeled data from the arXiv database, we train a baseline AI publication classifier with the SPECTER transformer language model that achieves 96\% accuracy.
    %
   
    %
    %This approach provides labels for a broader sample of scientific publications beyond arXiv, drawn from OpenAlex.
    %
    %A SPECTER model trained on this corpus achieves 97\% accuracy.
    %
    %Our results indicate that with effective prompt engineering, chatbots can be used as reliable data annotators even where subject-area expertise is required. Generating a dataset of GPT-labeled AI publications, we compare both classifiers on a set of publications from the top 13 AI conference venues to evaluate the utility of chatbots as data annotators for downstream tasks. 

\begin{comment}
    
    We train a baseline AI classification model using expert-labeled data from the arXiv database and the SPECTER transformer language model, which was fine-tuned for scientific text tasks. 

    
    Achieving 96\% accuracy using arXiv data, we experiment with prompt engineering to generate a chatbot-labeled dataset to train a new AI publication classifier with. 
    Using GPT models, we achieve 94\% accuracy on labeling publications as AI or non-AI based on their titles and abstracts. 
    Our results indicate that with effective prompt engineering, chatbots can be used as a reliable data annotator when subject-area expertise is required. 
\end{comment}        


\end{abstract}

==> 3_methodology/3_methodology.tex <==
\section{Experimental Design}
We design a framework to evaluate the utility of chatbots as expert annotators through prompt engineering and classification model performance, as shown in Figure \ref{fig:design}. Each step in this process can be adapted to a specific classification task, provided that there is a baseline labeled dataset or a comparable evaluation task for prompt engineering. In a small data task chatbot annotation could completely replace the classifier model. However, in this work we focus on tasks that use large datasets, which would be time-intensive and costly for a chatbot to annotate entirely.  

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{LaTeX/3_methodology/pipeline_flow_1.pdf}
\caption{Classification framework diagram}
\label{fig:design}
\end{figure}

\subsection{Scientific Publication Classifier}
We experiment with two publicly available transformer language models: SciBERT and SPECTER. SciBERT is a pre-trained language model based on the Bidirectional Encoder Representations from Transformers (BERT) model and trained on a sample of 1.14M papers from Semantic Scholar (using full-text) \cite{Beltagy2019SciBERT}. The Scientific Paper Embeddings using Citation-informed TransformERs (SPECTER) improves on SciBERT by incorporating the citation graph that exists between academic publications \cite{specter2020cohan}. Compared to SciBERT, SPECTER has proven to decrease training times while maintaining - if not exceeding - performance metrics, particularly for classification tasks.

We implement all scientific publication classifiers in the same way, changing transformer models and datasets for each experiment. Table \ref{tab:model_parameters} displays the non-default parameters that we set for our classification experiments. We use train, test, validation dataset splits of 70\%, 15\%, and 15\% respectively. 


\begin{table}[ht]
    \centering
    \begin{tabularx}{\columnwidth}{Xr}
         \toprule
         \textbf{Parameter} & \textbf{Value}  \\ \midrule
        \texttt{max\_train\_samples} & 30000 \\
        \texttt{max\_eval\_samples} & 10000 \\
        \texttt{max\_seq\_length} & 512 \\
        \texttt{evaluation\_strategy} & steps \\
        \texttt{eval\_steps} & 100 \\
        \texttt{per\_device\_train\_batch\_size} & 16 \\
        \texttt{per\_device\_eval\_batch\_size} & 16 \\
        \texttt{gradient\_accumulation\_steps} & 4 \\
        \texttt{tpu\_num\_cores} & 8 \\
        \texttt{bf16} & true \\
        \texttt{bf16\_full\_eval} & true \\
         \bottomrule
    \end{tabularx}
\caption{Training parameters for AI publication classification experiments}
\label{tab:model_parameters}
\end{table}



%Both classification models are implemented in the same way...\autumn{to fill}

\subsection{Data Annotation Prompt Engineering}
To automatically identify AI research publications we leverages state-of-the-art LLMs' chatbot feature to assign binary (AI or not-AI) labels given a publication's title and abstract. This requires experimentation in prompt engineering to select a prompt that will produce reliable labels that are usable on their own (e.g., treating the chatbot as the classifier) or functional for generating training data (e.g., creating a labeled dataset). We aim to identify a single, zero-shot prompt that will produce accurate and parsable responses to initiate an automated annotation pipeline. 

We use the GPT-3.5-Turbo and GPT-4 chatbots, as GPT-4 is a more robust model but consequently is significantly more costly to query; GPT-4 is approximately 20 times more expensive than GPT-3.5-Turbo. Using the \texttt{openai} Python package, we run our prompt engineering experiments with the parameters described in Table \ref{tab:gpt_parameters}. 

\begin{table}[ht]
    \centering
    \begin{tabularx}{\columnwidth}{Xr}
         \toprule
         \textbf{Parameter} & \textbf{Value}  \\ \midrule
         \texttt{model} & gpt-3.5-turbo, gpt-4 \\
        \texttt{temperature} & 0 \\
        \texttt{top\_p} & 0.1 \\
        \texttt{n} & 1 \\
        \texttt{stream} & False \\
        \texttt{presence\_penalty} & 0 \\
        \texttt{frequency\_penalty} & 0 \\
         \bottomrule
    \end{tabularx}
\caption{\texttt{openai.ChatCompletion} parameters for prompt engineering experiments.}
\label{tab:gpt_parameters}
\end{table}

We design a series of prompts that provide increasing specificity of the AI expertise we ask the GPT chatbot models to personify: a reader, a researcher, and a subject-matter expert. Table \ref{tab:prompts} lists the nine prompts that we test, with the first three prompts denoting the personas of varying levels of expertise. Each of the three personas are then tested with variations to the instructions, providing the chatbot with awareness of non-relevant publications and clarity on how to annotate. These prompts result in consistent and parsable responses, enabling us to compare their performance across chatbot models and prompts. 

\newcolumntype{R}{>{\raggedright\arraybackslash}m{5.9in}}
\begin{table*}[ht!]
    \centering
    \begin{tabularx}{\textwidth}{p{0.8in}R}
         \toprule
         \textbf{Prompt Type} & \textbf{Prompt}\\ \midrule
        Reader & You are \textbf{someone reading} in AI/ML, and you are given an annotation task. Given a publication's title and abstract, assign a AI or Non-AI label determining if the publication belongs to the field of AI/ML research and a predicted probability of relevance. Provide just the label and prediction in your answer. 
        
        \\
        Researcher & You are a \textbf{researcher} in AI/ML, and you are given an annotation task. Given a publication's title and abstract, assign a AI or Non-AI label determining if the publication belongs to the field of AI/ML research and a predicted probability of relevance. Provide just the label and prediction in your answer 
        
        \\
        Expert & You are a \textbf{subject-matter expert} in AI/ML, and you are given an annotation task. Given a publication's title and abstract, assign a AI or Non-AI label determining if the publication belongs to the field of AI/ML research and a predicted probability of relevance. Provide just the label and prediction in your answer. 
        
        \\
        Uncertainty & You are a \textbf{[persona type]} in AI/ML, and you are given an annotation task. Given a publication's title and abstract, assign a AI or Non-AI label determining if the publication belongs to the field of AI/ML research and a predicted probability of relevance. \textbf{Some papers may be in STEM fields but not exactly AI, please assign AI only if you are confident.} Provide just the label and probability in your answer. 
        
        \\
        Uncertainty and clarity &  You are a \textbf{[persona type]} in AI/ML, and you are given an annotation task. Based on the title and abstract of an academic publication, assign a label ‘AI’ or ‘Non-AI’ indicating whether the publication belongs to the field of AI/ML research. Also assign a score between 0 and 1 that describes how confident you are in the label. \textbf{Some papers may be in STEM fields but not exactly in AI/ML. Please assign the ‘AI’ label only if you are confident. Otherwise, assign the ‘Non-AI’ label and quantify your uncertainty in the score}. Respond only with the label and the score.\\

         \bottomrule
    \end{tabularx}
\caption{Zero-shot chatbot prompt variations for reliable data annotation experiments.}
\label{tab:prompts}
\end{table*}

In addition to asking for a label, we ask the chatbot to provide a predicted probability of relevance to further investigate the reliability of the responses. 

\subsection{Classifier Performance Evaluation}
We include an evaluation task that is separate from comparing the validation performance of the two classification models. This evaluation task should compute model performance on a new dataset to evaluate the generalizability of the models, as one goal of using chatbots for data annotation is generating a more representative training dataset. 

For our domain application, we follow \citet{toney2022multi} and use a set of publications that appeared in one of the 13 top AI and ML conferences from CSRankings\footnote{\url{csrankings.org}}:

\begin{enumerate}
\setlength{\itemsep}{0pt}
    \item AAAI Conference on Artificial Intelligence
    \item International Joint Conference on Artificial Intelligence
    \item IEEE Conference on Computer Vision and Pattern Recognition
    \item European Conference on Computer Vision
    \item IEEE International Conference on Computer Vision
    \item International Conference on Machine Learning
    \item International Conference on Knowledge Discovery and Data Mining
    \item Neural Information Processing Systems
    \item Annual Meeting of the Association for Computational Linguistics
    \item North American Chapter of the Association for Computational Linguistics
    \item Conference on Empirical Methods in Natural Language Processing
    \item International Conference on Research and Development in Information Retrieval
    \item International Conference on World Wide Web.
\end{enumerate}




%---OLD TEXT------------------------
\begin{comment}
    was trained on the full text of SemanticScholar’s corpus of scientific literature.

    We use SciBERT, a publicly available Bidirectional Encoder Representations from Transformers (BERT) model offered from the Allen Institute for AI (AllenAI). SciBERT was trained on the full text of SemanticScholar’s corpus of scientific literature. The relevant training set coupled with the model-specific vocabulary made SciBERT the best available choice in 2019.

     The relevant training set coupled with the model-specific vocabulary made SciBERT the best available choice in 2019

 In 2021, AllenAI released a new publicly-available model for determining document relatedness: Scientific Paper Embeddings using Citation-informed TransformERs (SPECTER).

  Rather than relying entirely on the semantics of a given publication’s title or abstract, SPECTER leverages the citation graph that exists between academic publications. Compared to SciBERT, SPECTER has proven to decrease training times while maintaining - if not exceeding - performance metrics. 

  One attempt to define AI/ML-relevant publications draws upon arXiv’s publicly available database of academic publications. Authors submit their publications to the site and manually label each according to arXiv’s research taxonomy. Each publication can receive multiple labels from the author, ensuring that any multidisciplinary research can be appropriately labeled.  
The project’s explicit definition of AI-relevant research is the union of six arXiv-defined subjects in computer science and statistics: artificial intelligence, computation and language, computer vision, machine learning, multi-agent systems, and robotics. The arXiv classifier is trained on titles and abstracts of these author-labeled arXiv publications. The results from the classifier are publications in which their predicted AI/ML-relevance is greater than 0.50. 
The first iteration of the arXiv classifier utilized 



This project utilizes OpenAI’s API to generate predictions of relevance based upon a publication’s title and abstract text using both GPT-3.5-Turbo and GPT-4. These pre-trained models offer much faster results than building a model from scratch, and leverage a wider corpus of training materials. GPT-3.5-Turbo has been optimized for chat and was trained using Reinforcement Learning from Human Feedback. GPT-4 is a large multi-modal model that has displayed stronger performance on a variety of simulated exams and performance benchmarks than GPT-3.5-Turbo. The resulting predictions are then tested on the author-generated labels from arXiv to derive evaluations. For completeness, multiple input prompts were tested to find the best performance for our labeling task. 


\begin{flushleft}
\textbf{GPT for Annotation}
\end{flushleft}

Another attempt to define AI/ML relevant research leverages state-of-the-art large language models (LLMs) to obtain labels for research publications. This project utilizes OpenAI’s API to generate predictions of relevance based upon a publication’s title and abstract text using both GPT-3.5-Turbo and GPT-4. These pre-trained models offer much faster results than building a model from scratch, and leverage a wider corpus of training materials. GPT-3.5-Turbo has been optimized for chat and was trained using Reinforcement Learning from Human Feedback. GPT-4 is a large multi-modal model that has displayed stronger performance on a variety of simulated exams and performance benchmarks than GPT-3.5-Turbo. The resulting predictions are then tested on the author-generated labels from arXiv to derive evaluations. For completeness, multiple input prompts were tested to find the best performance for our labeling task. 

\begin{flushleft}
\textbf{OpenAlex with GPT Labels SPECTER Classifier}
\end{flushleft}

Lastly, this project tests the efficacy of synthetic labels for classification tasks. Class imbalance represents a key limitation of using a crowd-sourced definition of AI/ML research from arXiv. Furthermore, arXiv offers just a solitary venue for learning a definition of AI/ML-relevance. This project tests the performance impact of leveraging GPT-generated labels for publications from OpenAlex relative to author-derived labels from arXiv for SPECTER-based models. This process measures the effect of combining labeling performance of LLMs with the learning capability of SPECTER. 

\end{comment}
